3D Line Mapping Revisited

In contrast to sparse keypoints, a handful of line segments can concisely encode the high-level scene layout, as they often delineate the main structural elements. In addition to offering strong geometric cues, they are also omnipresent in urban landscapes and indoor scenes. Despite their apparent advantages, current line-based reconstruction methods are far behind their point-based counterparts. In this paper we aim to close the gap by introducing LIMAP, a library for 3D line mapping that robustly and efficiently creates 3D line maps from multi-view imagery. This is achieved through revisiting the degeneracy problem of line triangulation, carefully crafted scoring and track building, and exploiting structural priors such as line coincidence, parallelism, and orthogonality. Our code integrates seamlessly with existing point-based Structure-from-Motion methods and can leverage their 3D points to further improve the line reconstruction. Furthermore, as a byproduct, the method is able to recover 3D association graphs between lines and points / vanishing points (VPs). In thorough experiments, we show that LIMAP significantly outperforms existing approaches for 3D line mapping. Our robust 3D line maps also open up new research directions. We show two example applications: visual localization and bundle adjustment, where integrating lines alongside points yields the best results. Code is available at https://github.com/cvg/limap.

==> figs/supp_qualitative_wo_citations.tex <==
\begin{figure*}
\scriptsize
\setlength\tabcolsep{2pt} % default value: 6pt
\begin{tabular}{ccc}
{\includegraphics[width=0.3\linewidth, height=114pt]{figs/imgs/qualitative_supp/british_museum2.png}} & 
{\includegraphics[width=0.3\linewidth, height=114pt]{figs/imgs/qualitative_supp/florence_cathedral_side3.png}} &
{\includegraphics[width=0.3\linewidth, height=114pt]{figs/imgs/qualitative_supp/london_bridge.png}} \\
\textit{British Museum} &
\textit{Florence Cathedral Side} &
\textit{London Bridge}
\\
{\includegraphics[width=0.3\linewidth, height=114pt]{figs/imgs/qualitative_supp/piazza_san_marco.png}} & 
{\includegraphics[width=0.3\linewidth, height=114pt]{figs/imgs/qualitative_supp/lincoln_memorial_statue.png}} &
{\includegraphics[width=0.3\linewidth, height=114pt]{figs/imgs/qualitative_supp/st_pauls_cathedral.png}}
 \\
\textit{Piazza San Marco} &
\textit{Lincoln Memorial Statue} &
\textit{St. Paul's Cathedral}
\\
{\includegraphics[width=0.3\linewidth, height=114pt]{figs/imgs/qualitative_supp/OldHospital.png}} & 
{\includegraphics[width=0.3\linewidth, height=114pt]{figs/imgs/qualitative_supp/StMarysChurch.png}} & 
{\includegraphics[width=0.3\linewidth, height=114pt]{figs/imgs/qualitative_supp/Auditorium.png}} \\
\textit{Old Hospital} &
\textit{St. Mary's Church} &
\textit{Auditorium}
\\
{\includegraphics[width=0.3\linewidth, height=114pt]{figs/imgs/qualitative_supp/Courtroom_outside.png}
\hspace{-0.09\linewidth}\includegraphics[width=0.09\linewidth]{figs/imgs/qualitative_supp/Courtroom_inside.png}} & 
{\includegraphics[width=0.3\linewidth, height=114pt]{figs/imgs/qualitative_supp/Truck.png}} & 
{\includegraphics[width=0.3\linewidth, height=114pt]{figs/imgs/qualitative_supp/Train.png}} \\
\textit{Courtroom} (indoor and outdoor) &
\textit{Truck} &
\textit{Train}
\\
{\includegraphics[width=0.3\linewidth, height=114pt]{figs/imgs/qualitative_supp/Lighthouse.png}} & 
{\includegraphics[width=0.3\linewidth, height=114pt]{figs/imgs/qualitative_supp/Museum.png}} & 
{\includegraphics[width=0.3\linewidth, height=114pt]{figs/imgs/qualitative_supp/Temple.png}} \\
\textit{Lighthouse} &
\textit{Museum} &
\textit{Temple}
\\
\end{tabular}
\centering
\caption{\textbf{More qualitative results of the 3D line maps recovered by our framework.}}
\label{fig::supp_qualitative}
\end{figure*}


==> figs/tmp_supp_qualitative_3x5.tex <==
\begin{figure*}
\scriptsize
\setlength\tabcolsep{2pt} % default value: 6pt
\begin{tabular}{ccccc}
{\includegraphics[width=0.19\linewidth, height=84pt]{figs/imgs/qualitative_supp/british_museum2.png}} & 
{\includegraphics[width=0.19\linewidth, height=84pt]{figs/imgs/qualitative_supp/florence_cathedral_side3.png}} &
{\includegraphics[width=0.19\linewidth, height=84pt]{figs/imgs/qualitative_supp/london_bridge.png}} &
{\includegraphics[width=0.19\linewidth, height=84pt]{figs/imgs/qualitative_supp/piazza_san_marco.png}} & 
{\includegraphics[width=0.19\linewidth, height=84pt]{figs/imgs/qualitative_supp/lincoln_memorial_statue.png}} \\
\textit{British Museum} &
\textit{Florence Cathedral Side} &
\textit{London Bridge} &
\textit{Piazza San Marco} &
\textit{Lincoln Memorial Statue}
\\
{\includegraphics[width=0.19\linewidth, height=84pt]{figs/imgs/qualitative_supp/st_pauls_cathedral.png}} &
{\includegraphics[width=0.19\linewidth, height=84pt]{figs/imgs/qualitative_supp/OldHospital.png}} & 
{\includegraphics[width=0.19\linewidth, height=84pt]{figs/imgs/qualitative_supp/StMarysChurch.png}} & 
{\includegraphics[width=0.19\linewidth, height=84pt]{figs/imgs/qualitative_supp/Auditorium.png}} &
{\includegraphics[width=0.19\linewidth, height=84pt]{figs/imgs/qualitative_supp/Truck.png}} \\
\textit{St. Paul's Cathedral} &
\textit{Old Hospital} &
\textit{St. Mary's Church} &
\textit{Auditorium} &
\textit{Truck}
\\
{\includegraphics[width=0.19\linewidth, height=84pt]{figs/imgs/qualitative_supp/Courtroom_outside.png}
\hspace{-0.09\linewidth}\includegraphics[width=0.09\linewidth]{figs/imgs/qualitative_supp/Courtroom_inside.png}} & 
{\includegraphics[width=0.19\linewidth, height=84pt]{figs/imgs/qualitative_supp/Train.png}} &
{\includegraphics[width=0.19\linewidth, height=84pt]{figs/imgs/qualitative_supp/Lighthouse.png}} & 
{\includegraphics[width=0.19\linewidth, height=84pt]{figs/imgs/qualitative_supp/Museum.png}} & 
{\includegraphics[width=0.19\linewidth, height=84pt]{figs/imgs/qualitative_supp/Temple.png}} \\
\textit{Courtroom} (indoor and outdoor) &
\textit{Train} &
\textit{Lighthouse} &
\textit{Museum} &
\textit{Temple}
\\
\end{tabular}
\centering
\caption{\textbf{More qualitative results of the 3D line maps recovered by our framework.}}
\label{fig::supp_qualitative}
\end{figure*}


==> tex/body.tex <==
\section{Introduction}

\input{tex/intro.tex}

\section{Related Work}

\input{tex/related_work}

\section{The Proposed 3D Line Mapping Pipeline}

\input{tex/reconstruction}

\section{Experiments}

\input{tex/experiments}

\section{Conclusion}

\input{tex/conclusion}


==> tex/experiments_shortened.tex <==
\label{sec::exp}
\noindent
\textbf{Implementation Details. }
Our whole library is implemented in C++ with Python bindings~\cite{pybind11}. The triangulation and scoring can be run in parallel for each node, enabling scalability to large datasets. We use $n_v = 20$ visual neighbors and keep the top $K = 10$ line matches. We provide all the values of thresholds and scaling factors in Sec. F.2 in supp.
% The scaling factors introduced in Section~\ref{sec:scoring} are set as follows: $\tau_a = 10$ deg for the angle in 3D and $\tau_a = 8$ deg in 2D, $\tau_o = 0.05$ for the overlap in 2D and 3D, $\tau_p = 5$ pixels for the perpendicular distance in 2D, and $\tau_s = 0.015$ for the scale-invariant endpoint distances in 3D. 
% Please refer to the supp. for more details.
% In 3D, we set the angle scaling factor $\tau_a = 10$ deg, and the one for scale-invariant endpoint distance to $\tau_p = 0.015$. For track association, the overlap threshold in both 3D and 2D is set to 0.05 and the \textit{InnerSeg} threshold is set to the minimum uncertainty between the pair. In 2D, the angle threshold is set to 8 degrees and the perpendicular distance threshold is set to 5 pixels. Please refer to the supp. for more details.
% \todo{Add the thresholds $t_f = 1$ and $t_m = 0.5$  (but the scaling factors get stricter) to prune edges in track building and to merge tracks.}

\subsection{Line Mapping}

\input{tabs/main_hypersim}
\input{tabs/main_tnt}

To validate the effectiveness of our system, we set up an evaluation benchmark to quantify the quality of the reconstructed 3D line maps. As there are no ground truth (GT) 3D lines, we evaluate the 3D line mapping with either GT mesh models or point clouds. We use the following metrics:
\begin{itemize}[noitemsep,nolistsep]
    \item \textit{Length recall} (in meters) at $\tau$ ($R
\tau$): sum of the lengths of the line portions within $\tau$ mm from the GT model.
    \item \textit{Inlier percentage} at $\tau$ ($P
\tau$): the percentage of tracks that are within $\tau$ mm from the GT model.
    \item \textit{Average supports}: average number of image supports and 2D line supports across all line tracks.
\end{itemize}

In the following, we compare our system with two state-of-the-art methods as baselines: L3D++ \cite{hofer2017efficient} and ELSR \cite{wei2022elsr}, using two line detectors: the traditional LSD detector \cite{von2008lsd} and the learning-based SOLD2 \cite{pautrat2021sold2}. For ELSR \cite{wei2022elsr}, we convert the input into VisualSfM \cite{wu2011visualsfm} format and use code\footnote{\texttt{https://skyearth.org/publication/project/ELSR/}} from the authors (only supporting LSD \cite{von2008lsd}).

Our first evaluation is run on the first eight scenes of the Hypersim dataset \cite{roberts:2021}, composed of 100 images each, and is reported in \cref{tab::main-hypersim}.
For both detectors, we reconstruct much more complete line maps with better or comparable precision than the competitors, while also exhibiting significantly higher quality of track information. This abundant track association is beneficial particularly for line-based applications such as visual localization \cite{gao2022pose}.
%We also double checked with the authors. ELSR \cite{wei2022elsr} does not achieve satisfactory results probably due to lack of point and plane features, but its contribution has potential to be integrated into our system to improve the matches.
After discussing with the authors of ELSR, it seems that their method does not achieve satisfactory results due to a lack of point and plane features.
% However, their new matching scheme is orthogonal to our method and could in principle be used as a drop-in replacement for scenes where they perform well.
%and it is possible that for scenes where it does improve, their matching scheme could in principle be integrated into our system. 

\input{figs/tnt_comparison}
\input{figs/qualitative}

We further evaluate all three methods on the \textit{train} split of the \textit{Tanks and Temples} dataset~\cite{Knapitsch2017} without \textit{Ignatius} as it has no line structures. As SOLD2 \cite{pautrat2021sold2} is trained for indoor images, we only use LSD \cite{von2008lsd}. Since the provided point cloud was cleaned to focus only on the main subject, we compute its bounding box, extend it by one meter, and only evaluate lines inside this region. This prevents incorrectly penalizing correct lines that are far away from the main scene, which our method is particularly good at thanks to our scale-invariant design (refer to Sec. G in supp.). \cref{tab::main-tnt} shows the results, where our methods significantly improve the mapping quality across the board. \cref{fig::tnt_comparison} shows qualitative comparison between our method and L3D++ \cite{hofer2017efficient}. Our results exhibit better completeness, have less noisy lines that are flying around, and achieve significantly more robust reconstructions of subtle details (e.g. on the ground). More examples of our produced line maps are shown in \cref{fig::qualitative}.

\input{figs/qualitative_structures}

As an additional output of our system, junction structures and line-line relations such as parallelism and orthogonality are discovered, as shown in \cref{fig::qualitative_structures}. This directly comes from the line-point and line-VP soft associations of \cref{sec:refinement}. From the recovered structures, we can clearly perceive the scene and easily recognize the main Manhattan directions \cite{coughlan2000manhattan}.
% , which is a new step towards building structured 3D maps that align better with human perception of the building layout.

\input{figs/scalability}

To demonstrate the scalability of the proposed system, we also run our method on two large-scale datasets: Aachen (6,697 images) \cite{sattler2012image,sattler2018benchmarking} and Rome city (16,179 images) \cite{snavely2006photo,snavely2008modeling,agarwal2011building}. \cref{fig::scalibility} shows that our method produces reliable line maps with clear structures. Note that the camera poses from Bundler \cite{snavely2006photo} on Rome city are far from perfect, while our mapping still works reasonably well. The efficiency bottleneck is in line detection and matching (we use SOLD2 \cite{pautrat2021sold2} descriptors), while the rest of the mapping takes only $\sim$10 minutes on Aachen \cite{sattler2012image,sattler2018benchmarking}.
The time complexity of our system is nearly linear with the number of images. 

\subsection{More Insights and Ablation Studies}

\input{figs/adelaidermf}
\input{tabs/ablations_endpoints}
\input{tabs/ablations_triangulation}

\noindent
\textbf{Line Triangulation.} To study the stability of the triangulation, we perform a small test on a stereo pair from AdelaideRMF \cite{AdelaideRMF} on the uncertainty (measured by the largest singular value of the covariance) of the triangulated 3D segments. We further run a synthetic experiment by generating random lines on a plane orthogonal to the stereo pair, and plot the uncertainty of point and line triangulations with respect to the angle of the lines with the baseline (refer to Sec. D in supp. for details). The results in \cref{fig::synthetic_tests} show that when the matched line is nearly parallel to the epipolar line, the line triangulation becomes degenerate with exploding uncertainty, while triangulating the endpoints is significantly more stable. Thus, combining points and VPs from the 2D association is beneficial to improve the stability of the proposals. However, the endpoints are generally not consistent across line matches in practice and need to be complemented with line-line triangulation. This can be verified in \cref{tab::ablations_endpoints} where the performance significantly drops when we change line triangulation into endpoint triangulation.

We further ablate our four types of triangulation for generating proposals. Results in \cref{tab::ablations_triangulation} show that integrating points and VPs enhance the 3D line maps, in particular significantly improving the track quality. Another surprising fact is that the third line in the table, relying only on points and line + point triangulation, already achieves better results than the prior baselines in \cref{tab::main-hypersim}. Employing all four types of proposals obtains the best trade-off.

\input{tabs/ablations_line3dpp}

\noindent
\textbf{Scoring and Track Building.}
We first study the effects of using exhaustive line matching as in L3D++ \cite{hofer2017efficient}. To enable direct comparison we only use line triangulation proposals. Results are shown in \cref{tab::ablations_matcher}. While there are more proposals generated from the exhaustive matches, both the recall and precision decrease by a noticeable margin. This is probably due to the large number of wrong proposals misleading the scoring process. Nevertheless, our method with exhaustive matches still works significantly better than L3D++ \cite{hofer2017efficient}. To further study the effects of the proposed distance measurements at scoring and track building (merging), we re-implement the ones proposed in L3D++ \cite{hofer2017efficient} and perform direct comparison. Both our scoring and track building are significantly better, especially when equipped with SOLD2 \cite{pautrat2021sold2} which produces more structured lines. 

\noindent
\textbf{Joint Optimization.}
\input{tabs/ablations_refinement}
Finally, we ablate the proposed joint optimization in our pipeline. First, we remove the point-line association and only apply the geometric residuals (reprojection error). Results in \cref{tab::refine-hypersim} show that the geometric refinement improves significantly when the proposals solely come from line triangulation. However, when adding additional proposals from points and VPs, it contributes marginally and even misleads some lines that are generated from points and VPs but poorly conditioned for lines (R10 decreases). When integrated with joint optimization with soft association, the recall is further improved noticeably, while sacrificing a bit on the precision. It is worth pointing out that the joint optimization also enables the byproduct of junction structures and line-line relations (e.g. in \cref{fig::qualitative_structures}).

\subsection{Applications}

\input{tabs/localization.tex}
\input{figs/localization_with_table}

\noindent
\textbf{Line-Assisted Visual Localization.}
We build a hybrid visual localization with both points and lines on top of the acquired 3D line maps. Specifically, we first build point maps as in HLoc \cite{sarlin2019coarse,hloc} and line maps with our proposed method. Then, we match points and lines respectively and get 2D-3D correspondences from the track information in the 3D maps. Given these correspondences, we combine four minimal solvers \cite{kukelova2016efficient,persson2018lambda,zhou2018stable}: P3P, P2P1LL, P1P2LL, P3LL from PoseLib \cite{PoseLib}, together in a hybrid RANSAC framework \cite{camposeco2018hybrid,Sattler2019Github} with local optimization \cite{chum2003locally,Lebeda2012BMVC} to get the final 6-DoF pose (refer to Sec. H in supp. for details). This also enables direct comparison since only using P3P \cite{persson2018lambda} corresponds to the point-alone baseline similar to HLoc \cite{sarlin2019coarse,hloc}. We also compare with the post-refinement of PtLine \cite{gao2022pose} that optimizes over the initial point-alone predictions.

Results in \cref{tab:localization} show that our localization system achieves consistently better results than the point-alone baseline both indoors \cite{7scenes} and outdoors \cite{kendall2017geometric}, validating the effectiveness of employing 3D line maps for visual localization. 
In \cref{fig::stairs} we show more detailed results from the \textit{Stairs} scene from 7Scenes~\cite{7scenes} as it is one of the most challenging ones. Integrating lines significantly benefits the alignment of the reprojected structures, improving the pose accuracy from 46.8 to 71.1. Also, with our localization pipeline, using the map built from our proposed method is better than from L3D++ \cite{hofer2017efficient} by a noticeable margin, again demonstrating the advantages of our proposed line mapping system. 

\noindent
\textbf{Refining Structure-from-Motion.}
\input{tabs/sfm_hypersim}
With the acquired 3D line maps built from a roughly correct point-based structure-from-motion model, e.g, COLMAP \cite{schonberger2016structure}, we can use the 3D lines with their track information to refine the input camera poses with joint optimization of points and lines. To verify this, we run COLMAP \cite{schonberger2016structure} with SuperPoint \cite{detone2018superpoint} on the first eight scenes of Hypersim \cite{roberts:2021}, run the proposed line mapping on top of it, and perform joint bundle adjustment to refine poses and intrinsics.
We report the relative pose evaluation of all image pairs~\cite{jin2021image}.
\cref{tab:sfm_hypersim} shows that the joint point-line refinement consistently benefits the accuracy of the camera poses, in particular improving AUC@1$^\circ$ by 5.6.




==> tex/rebuttal.tex <==
\definecolor{custom_red}{rgb}{0.8500,0.3250,0.0980}%
\definecolor{custom_green}{rgb}{0.4660,0.6740,0.1880}%
\definecolor{custom_blue}{rgb}{0,0.4470,0.7410}%
\newcommand{\rone}{{\color{custom_red} \textbf{3KFH}}}
\newcommand{\rtwo}{{\color{custom_green} \textbf{zWFi}}}
\newcommand{\rthree}{{\color{custom_blue} \textbf{t5yk}}}
\noindent We thank all reviewers for their constructive feedback, and appreciate all the positive comments. We here promise again that the full implementation of the LIMAP library, including all stages of mapping, evaluation, hybrid localization, and joint bundle adjustment, will be released upon publication, with Python bindings available to ensure the flexibility to change modules such as line detectors and matchers.
%, to benefit future development of the relevant practices.
Below we answer specific reviewer comments.

%Please see below our response to specific comments. 

% (\textbf{R1:} \rone; \textbf{R2:} \rtwo; \textbf{R3:} \rthree)

\noindent
\textbf{\rone: Exploiting statistical properties. }
We really appreciate all the constructive comments which are extremely helpful to us and we will try to improve the paper accordingly. Employing uncertainty measurement at filtering proposals, measuring distances, and aggregation is conceptually reasonable and indeed very helpful in our experiments. One concern is that storing 6x6 covariances for each proposal largely increases the storage needed (the proposals are currently the bottleneck for the storage) and uncertainty propagation also requires additional overhead, so we keep the strategy simple in the current design to ensure scalability to large datasets. Nevertheless, we have been making efforts to integrate the uncertainties in the next iteration of the code and will provide our interface for covariance estimation (as in Section D in supp.) in the released library. Regarding the bundle adjustment, the Ceres-based implementation uses local parameterizations in each iteration to ensure we only optimize over 4-DoF for each line, so there are no extra Lagrange multipliers included.

%Regarding bundle adjustment, the Ceres parameterization we used shares similar spirits with the recommended literature by using iterative updates, which does not involve integration of the Lagrangian. \todo{double check? improve this? Mahalanobis distance?}

\noindent
\textbf{\rone: How large are the models in mm? }
We will update the paper to more clearly include the size of the scenes for comparison. Most scenes in the paper are around 5~-~20 m in diameter (excluding some of the larger ones, e.g.~Aachen). The length recall reported in all tables are in meters.

%The scales in both datasets are aligned to those in real life (i.e. around 5-20 meters). The length recall reported in all tables are in meters. We will make it clearer in the revision.

\noindent
\textbf{\rone: Advantages of using line features from the pixel standard deviation perspective. }
Thank you for the suggestion. We totally agree and will add it to the introduction.

\noindent
\textbf{\rtwo: Extension to curved edges. }
While reconstructing general curves is also interesting, it is a much harder problem. Both in terms of detecting them in 2D, and finding a suitable parameterization in 3D for triangulation.


%First problem is to decide how to parameterize curves in 3D, and then 

%We would leave this interesting direction as future work.


%In the paper we focused on 3D line segments as 

%Our system focuses on reliable sparse features such as points, lines, planes, and their relations.
%While reconstructing general curves is also interesting, it is a much harder problem.  We would leave this interesting direction as future work.

%Both in terms of detecting them in 2D as finding a suitable parameterization in 3D. We would leave this interesting direction as future work.

%An extension to curved edges requires a new parameterization and a robust curve edge detector, and may require more than two views for triangulation. We would leave this interesting direction as future work.

\noindent
\textbf{\rtwo: Advanced VP estimation methods. }
Thank you for the suggestion. Integrating more advanced VP methods is not only helpful to the system but could also be valuable as a way to benchmark different methods. We decided to use JLinkage in the paper mainly for its simplicity and will include and discuss other VP methods in the final version.

\noindent
\textbf{\rthree: Ablation on the effects of scene points. }
The optional scene points can help improve the line maps on two stages: triangulation and joint optimization, and also enable the relational graph (Figure 6) as additional output. In all the experiments and ablations, ``Ours (line-only)" refers to our system without scene points, while the rest refers to our full system. The effects of scene points on triangulation and joint optimization are shown in Table 4 (bottom row vs. top row) and Table 6 (``joint optimization" vs. ``geom alone") respectively. While our system without scene points already works reasonably well, integrating scene points can further benefit the length recall and the number of supports, which is crucial to applications such as visual localization. We will make the description and analysis clearer in the revision.

\begin{figure}[tb]
\begin{center}
\begin{minipage}{\linewidth}
\begin{tabular}{@{}cc@{}}
    \renewcommand{\arraystretch}{0.6}
    \begin{tabular}[t]{@{}cc@{}}
    % \centering
        \raisebox{-\height}{\includegraphics[width=0.25\textwidth]{figs/imgs/rebuttal/MH1_1_lsd.png}} \\
        \raisebox{-\height}{\includegraphics[width=0.25\textwidth]{figs/imgs/rebuttal/MH1_5_lsd.png}} \\
        \raisebox{-\height}{\scriptsize LSD detections}
    \end{tabular}
    \raisebox{-0.88\height}{\includegraphics[width=0.66\textwidth]{figs/imgs/rebuttal/orbslam-fig1.png}} & 
\end{tabular}
\end{minipage} 
\vspace{-5pt}
\caption{Line mapping with ORB-SLAM3 on EuRoC MH01.}
\label{fig::rebuttal_orbslam}
\vspace{-26pt}
\end{center}
\end{figure}

% \begin{figure}[tb]
% \small
% \includegraphics[width=0.70\columnwidth, height=100pt]{figs/imgs/rebuttal/orbslam-fig1.png}
% \centering
% \caption{\scriptsize Our line mapping with ORB-SLAM3 on EuRoC MH01.}
% \label{fig::rebuttal_orbslam}
% \vspace{-20pt}
% \end{figure}

\noindent
\textbf{\rthree: Employing the poses and scene points of SLAM as alternative inputs to LIMAP over SfM.}
LIMAP requires as input a set of images, together with their camera poses. Optionally, a set of 2D points and their 3D tracks can be leveraged to provide 2D-3D point correspondences, which are beneficial to point-assisted triangulation, joint optimization, and BA. Both SfM and SLAM pipelines meet these requirements and can be used with LIMAP. The difference between the two is mainly the quality of the poses, which may be of a lower quality for SLAM. However, LIMAP is able to deal with noisy poses (e.g. from Bundler) and can even improve on top of them with joint BA (Table 8). 
Figure \ref{fig::rebuttal_orbslam} shows an example of LIMAP used with ORB-SLAM3 on the first scene of EuRoC. While the SLAM poses are noisier, we manage to triangulate a reasonable map of 3D lines.
% triangulate a larger number of lines.

%Thus, as long as SfM or SLAM is not failing, LIMAP can work with both inputs. Figure \ref{fig::rebuttal_orbslam} shows an example with LIMAP used on ORB-SLAM3 poses on the EuRoC dataset.


%Thus, as long as SfM or SLAM is not failing, LIMAP can work with both inputs, with a potential small drop of performance for SLAM poses. Figure \ref{fig::rebuttal_orbslam} shows an example with ORB-SLAM3 poses.

% In our mapping system, we assume that the camera pose for each image is available. This could come from SfM, SLAM or other alternatives that reliably estimate the poses. Our code release will support input poses from popular SfM systems [58,61,75]. While we show that LIMAP is able to deal with noisy poses (e.g. from Bundler) and can even improve on top of it with joint BA (Table 8), the input poses need to be roughly correct to support the mapping process, i.e. the mapping would not work if SfM/SLAM fails. It is true that the accuracy of camera poses from SfM and SLAM can be different sometimes, but this is beyond the scope of this paper as the required input of LIMAP can be any workable system that provides the pose for each image. Regarding the scene points as the additional input, what is required from LIMAP is the 3D point tracks that can provide 2D-3D point correspondences, which are beneficial to point-assisted triangulation, joint optimization and BA. The SLAM scene points, generally with their maps associated to keyframes and regular frames through registration and tracking, meet the requirement and can provide available 2D-3D point correspondences. Thus, they can be used for LIMAP, though the quality of the reconstructed point tracks from SLAM are generally not as good as the ones from SfM. \todo{improve this? maybe shorten this? this does not deserve that long}

\noindent
\textbf{\rthree: How to triangulate 3D point tracks from matched endpoints/junctions?}
Given matches over endpoints/junctions across a set of posed images, one can use standard 3D point triangulation methods. In our implementation we use the triangulation code from COLMAP.

%Given matches over endpoints/junctions across a set of posed images, one can efficiently perform triangulation to get 3D point tracks. We employ \textit{point\_triangulator} from COLMAP here.

\noindent
\textbf{\rthree: L3D++ and its implementation.}
Line3D++ is referred as L3D++ in our paper (Line 189). We did use their official implementation from GitHub (Line 1005 in supp.). As discussed in Section F.5 in supp., we updated two hyperparameters to enable fair comparison and also provided results with the default ones at Tabs. 3 and 4 in supp.  

\noindent
\textbf{\rthree: Integration of the new line detector DeepLSD.}
Thank you for the suggestion. We have integrated the open-source code of DeepLSD and it indeed works very well with LIMAP. DeepLSD + SOLD2 matcher scores 71.4 / 72.5 / (16.3 / 20.8) on ``R1 / P1 / \#supports" on Hypersim, being much better compared to 48.3 / 59.2 / (15.8 / 19.1) for LSD. It actually surpasses all the compared detectors by a large margin and achieves the best trade-off (detailed numbers can be found in Table 5 in our supplementary material).


==> tex/related_work.tex <==
\label{sec::related_work}
\noindent
\textbf{Line Detection and Matching. }
Detecting 2D line segments conventionally relies on grouping image gradients 
\cite{von2008lsd,akinlar2011edlines}. To improve the robustness and repeatability, learning-based line detectors were later proposed to tackle the problem of wireframe parsing \cite{huang2018learning,zhou2019learning,xue2019learning,zhang2019ppgnet,xue2020holistically,meng2020lgnn}. Recent deep detectors \cite{huang2020tp,pautrat2021sold2,xu2021line} manage to achieve impressive results for detecting general line segments. Matching of the detected line segments is often based on comparing either handcrafted \cite{bay2005wide,wang2009msld,zhang2013efficient,verhagen2014scale} or learning-based \cite{lange2019dld,vakhitov2019learnable,pautrat2021sold2,yoon2021line,abdellali2021l2d2} descriptors. Some recent methods also exploit point-line \cite{fan2010line,fan2012robust} and line-junction-line structures \cite{li2014robust,li2016hierarchical} to improve matching results, yet still not reaching the reliability level of advanced point matchers \cite{sarlin2020superglue,sun2021loftr}. Our method can leverage any line detector and matcher, and is robust to outliers.

~\\
\noindent
\textbf{Line Reconstruction.}
As a seminal work, Bartoli and Sturm \cite{bartoli2004framework,bartoli2005structure} proposed a full SfM pipeline for line segments, later improved by Schindler \cite{schindler2006line} with Manhattan-world assumption \cite{coughlan2000manhattan}. 
Jain et al. \cite{jain2010exploiting} proposed to impose global topological constraints between neighboring lines, which were further explored in \cite{ramalingam2015line,ranade2018novel,ren2021intuitive} to build wireframe models. Some learning-based methods \cite{zhou2019learning,luo2022LC2WF} were introduced as well to predict 3D wireframes. Hofer et al. \cite{hofer2014improving,hofer2015line3d,hofer2017efficient} proposed checking weak epipolar constraints over exhaustive matches and graph clustering, and introduced the Line3D++ software (referred as L3D++ in this paper), which remains the top choice \cite{gao2022pose,luo2022LC2WF} for acquiring 3D line maps so far. Recently, ELSR \cite{wei2022elsr} employed planes and points to guide the matching. However, all prior work mainly shows qualitative results and provides quantitative evaluation only on relatively small image sets \cite{strecha2008benchmarking,jain2010exploiting}. In this paper, we set up a quantitative evaluation on benchmarks with hundreds of images, where our proposed system significantly surpasses prior work by improving all stages in the mapping pipeline.

~\\
\noindent
\textbf{Line-based Applications.}
The resulting 3D line maps can be used for many downstream applications. \cite{hofer2017efficient} advocates the complementary nature of line reconstruction for structure visualization. Some incremental line-based SfM systems are introduced in \cite{zhang2014structure,micusik2017structure,holynski2020reducing}. To improve quality and robustness, recent methods \cite{zuo2017robust,pumarola2017pl,he2018pl,gomez2019pl,wei2019real,lim2021avoiding,lim2022uv} jointly employ point and line features in SLAM. While their line maps are often noisy and incomplete, noticeable improvement has been achieved in the accuracy of the recovered camera motion. There has also been development on VP estimation \cite{bazin_cvpr_2012,zhang2015,Li_2019_ICCV,Qian2022ARO} and solvers for joint point-line pose estimation \cite{ramalingam2011pose,vakhitov2016accurate,zhou2018stable,agostinho2019cvxpnpl}. Recently, promising performance in visual localization has been achieved by combining point and line features in a refinement step~\cite{gao2022pose}. In this paper, we show that our line maps can benefit multiple applications such as localization, SfM, and MVS (Sec. J in supp.). In particular, we present very competitive results on point-line visual localization.

\input{figs/overview}

